Estimating Information Flow in Deep Neural Networks

We study the flow of information and the evolution of internal representations during deep neural network (DNN) training, aiming to demystify the compression aspect of the information bottleneck theory. The theory suggests that DNN training comprises a rapid fitting phase followed by a slower compression phase, in which the mutual information $I(X;T)$ between the input $X$ and internal representations $T$ decreases. Several papers observe compression of estimated mutual information on different DNN models, but the true $I(X;T)$ over these networks is provably either constant (discrete $X$) or infinite (continuous $X$). This work explains the discrepancy between theory and experiments, and clarifies what was actually measured by these past works. To this end, we introduce an auxiliary (noisy) DNN framework for which $I(X;T)$ is a meaningful quantity that depends on the network's parameters. This noisy framework is shown to be a good proxy for the original (deterministic) DNN both in terms of performance and the learned representations. We then develop a rigorous estimator for $I(X;T)$ in noisy DNNs and observe compression in various models. By relating $I(X;T)$ in the noisy DNN to an information-theoretic communication problem, we show that compression is driven by the progressive clustering of hidden representations of inputs from the same class. Several methods to directly monitor clustering of hidden representations, both in noisy and deterministic DNNs, are used to show that meaningful clusters form in the $T$ space. Finally, we return to the estimator of $I(X;T)$ employed in past works, and demonstrate that while it fails to capture the true (vacuous) mutual information, it does serve as a measure for clustering. This clarifies the past observations of compression and isolates the geometric clustering of hidden representations as the true phenomenon of interest.

==> Sections/888-Comments.tex <==
% ==========================================================
% ICLR2019main.tex - Abstract
% ==========================================================

%We study the evolution of internal representations during training and the flow of information in deep neural networks (DNNs), aiming to demystify the compression aspect of the information bottleneck theory. The theory suggests training comprises a rapid ``fitting'' phase followed by a slower ``compression'' phase during which the mutual information $I(X;T)$ between the input $X$ and internal representation $T$ gradually decreases. While compression of \emph{the estimated mutual information} was observed by different groups of authors and in several DNN models, the true $I(X;T)$ over these DNNs is provably either constant (discrete $X$) or infinite (continuous $X$). This work explains the source of this inconsistency between theory and experiments and clarifies what was actually measured by these previous works. To do so, we introduce an auxiliary (noisy) DNN framework for which $I(X;T)$ is a meaningful quantity that depends on the network's parameters. Upon demonstrating that the proposed noisy framework is a good proxy for the original (deterministic) DNN of interest both in terms of performance and the learned representations, we first study $I(X;T)$ in this noisy regime. A rigorous estimator for $I(X;T)$ is developed, which enables tracking the evolution of this mutual information during training. We find that $I(X;T)$ indeed compresses in several noisy DNNs we examined. More importantly, however, by relating $I(X;T)$ over the noisy DNN to an information-theoretic communication problem, we show that compression is driven by the progressive clustering of hidden representations of inputs from the same class. Several methods to directly monitor clustering of hidden representations (applicable both in noisy and deterministic DNNs) are proposed, and used to demonstrate that although $I(X;T)$ is vacuous in deterministic DNNs, meaningful clusters are forming in the $T$ space nonetheless. As a last step, we circle back to the estimator of $I(X;T)$ employed in past works, and demonstrate that while it fails to capture the true (vacuous) mutual information, it does serve as a measure for clustering. This clarifies the past observations of compression and isolates the geometric clustering of hidden representations as the true phenomenon of interest.

\begin{comment}
\textbf{Color Menu:} I will use [\textsc{colored uppercase text in square brackets}] to leave comments in the text for each of us. The colors are: \brian{Brian}, \ewout{Ewout}, \igor{Igor}, \kristjan{Kristjan}, \nam{Nam}. If I need help writing certain parts of a section/subsection, I will indicate the person's name in the title (doing this gives a compilation warning, but one these are removed the warnings will go away). 

\textbf{Left To-Do:}
\begin{enumerate}
    \item First paragraph in the introduction. \kristjan{Kristjan}
    \item Experimental paragraph in the introduction. \brian{Brian -- pending the completion of the main experimental section}
    \item Experimental section - also talk about weight normalization and how it eliminated compression. Our interpretation is: normalization discourages clustering and forces the Gaussians means to spread out in space, which means MI in not dropping as much (if at all) \brian{Brian}\igor{Igor}\nam{Nam}
    \item Add Monte Carlo numerical integrated entropy value to experimental plots.  \brian{Brian}\igor{Igor}\nam{Nam}
    \item For Tishby's 3D layer (last) show the 3-dimensional box with the Gaussians mean for `important' epochs in training where something changes in the MI trajectory and explain each constellation causes MI to rise/fall.\igor{Igor}
    \item Last remark in estimation section showing some plots of SP-estimator and discussing it's pros compared to generic (kNN, KDE) estimators - better scaling with dimensionality, which is one of the most important facts for us. \kristjan{Kristjan}
    \item Tanh vs ReLU comparison subsection in the example section. \ewout{Ewout}
    \item Decide about inclusion of interpretation of the ICLR results ($\beta$-smoothed MI) in supplementary material. If included - it needs to be rewritten. \kristjan{Kristjan}
    \item Make the main paper fit into 8 pages.
    \item Polish the text.
\end{enumerate}
\end{comment}

%\section{Supplementary Material \textcolor{Magenta}{[\textsc{Will be separated for final version}]}}\label{SEC:Supplementary}

%\subfile{NIPS2018/Sections/Supplementary}

%Is this still relevant "clustering can be caused by multiple factors not limited to saturation, one of which is dimensionality reduction (e.g., in the linear SZT model)."


% \item clustering can be observed in higher dimensional neural networks, while clustering disappears due to the curse of dimensionality.
%\end{inparaenum}



\begin{comment}
in the context of a proposed noisy DNN model, for which the relevant mutual information is nontrivial. Through this rigorous formulation we developed a mutual information estimator tailored for noisy DNNs and derived convergence guarantees for it. We explored the compression aspect of IB theory, applying a communication channel perspective to explain various observed information compression patterns and relate them to underlying data clustering trends. Finally, we studied information trends in several small practical networks. %, observing similar overall trends. 
Our experiments showed that
\begin{inparaenum}[(i)]
\item compression directly relates to how spread out or clustered the data points are in a given layer, and
\item clustering can be caused by multiple factors not limited to saturation, one of which is dimensionality reduction (e.g., in the linear SZT model).
\item clustering can be observed in higher dimensional neural networks, while clustering disappears due to the curse fo dimensionality.
\end{inparaenum}
\end{comment}

%\kristjan{Would be good to have a unified ``declaration'' regarding compression and IB theory generally. Is it true? is it meaningful? should people pursue it? Or is compression just a thing that happens sometimes depending on initialization?}


% ==========================================================
% 1-Introduction
% ==========================================================

\begin{comment}

\textbf{point for intro:}
\begin{enumerate}
    \item detDNNs MI is constant -- no need to estimate it since it is just H(X) (or infinity if X is continuous).
    \item Still binning-based MI estimators over these detDNNs (which clearly fail to capture the true I(X;T) unless bin sizes --> 0) are showing compression. So what does it mean??
    \item Lets start with a framework where MI actually makes sense -- noisy DNNs. For these noisy DNNs, lets develop rigorous tools for tracking MI and check if compression (of the true MI over a noisy DNN) actually happens... If we see it (which we do), we can vouch that this is the true MI compression and not some artifact of estimation error. The reason we can vouch for it is our theoretical guarantees for SP MI estimator.
    \item OK, now we know that in noisy DNNs MI compresses (at least in some cases), but why does this happen? What are the underlying dynamics of the inner representations that cause this phenomena? This is where we get to the coalescing Gaussians observation, via Ewout's minimal example(s).
    \item Next step, still for noisy DNNs, we check that this coalescing Gaussians phenomena, aka clustering of representations, actually happens for larger noisy DNNs. This is what your noisy Tishby experiments are showing.
    \item Back to deterministic DNNs, we ask if clustering is an artifact of noise of something broader that happens? Well, although MI is now constant and thus meaningless, another way to understand the binning-based MI estimator is as a measure of clustering (verify this for noisy DNNs first comparing to the true estimated MI and seeing that the two are indeed correlated). When using this measure of clustering for deterministic DNNs we see  its compression (not compression of MI but just that I(X;Bin(T)) small <=> more clustered representations), which explains what previous works were actually observing: not MI compression, but increased clustering of representations.
\end{enumerate}
\end{comment}

%In recent years, deep neural networks (DNNs) achieved wide success in various complex classification tasks, including computer version, speech, and natural-language processing \ziv{references}. Yet, despite their empirical success, a theoretical understanding of DNNs is still largely lacking.

%\brian{Do we need to distinguish notation between noisy layer $T_\ell$ and deterministic layer $T_\ell$ for the abstract, intro and summary?}


%Recent work by \citet{DNNs_Tishby2017} studies the dynamics of DNN learning from an information-theoretic framework called the information bottleneck (IB) \citep{tishby_IB1999,tishby_DNN2015}. The framework considers the mutual information $I(X;T_\ell)$ between input $X$ and hidden layers $T_\ell$, and $I(Y;T_\ell)$ between the hidden layers and label $Y$. Plotting these quantities in two dimensions as they evolve during training produces a visualization of the optimization process in the ``information plane''. An interesting claim of \cite{DNNs_Tishby2017} is that while $I(Y;T_\ell)$ remains mostly constant as the layer index $\ell$ increases, the value of $I(X;T_\ell)$ decreases, suggesting that layers gradually shed irrelevant information about $X$. Moreover, they observed that after an initial fitting phase, there is a long compression phase during which $I(X;T_\ell)$ slowly decreases. It was suggested that this compression is responsible for the impressive generalization performance of DNNs. In a follow-up paper, \cite{DNNs_ICLR2018} contend that compression is not inherent to DNN training, claiming double-sided saturating nonlinearities, like tanh or sigmoid, yield compression while single-sided or non-saturating ones like ReLU do not necessarily compress. 

%\ziv{Point 1: MI is meaningless in detDNNs \& past plots are not showing MI}

%good to go?


%For instance, $T_\ell=\phi(\mathrm{W}_\ell T_{\ell-1}+b_\ell)+Z_\ell$ for fully connected or convolutional layers, where $\phi$ is the nonlinearity which operates on a vector component-wise, $\mathrm{W}_\ell\in\mathbb{R}^{d_\ell\times d_{\ell-1}}$ is the weight matrix and $b_\ell\in\mathbb{R}^{d_\ell}$ is the bias. 



%Our results do not rely on any particular~structure of $\{f_\ell\}_{\ell\in[L]}$, which can represent various types of layers (fully connected, convolutional, max-pooling, etc.). For instance, $T_\ell=\phi(\mathrm{W}_\ell T_{\ell-1}+b_\ell)+Z_\ell$ for fully connected or convolutional layers, where $\phi$ is the nonlinearity (e.g., $\tanh(x)$ or $\mathrm{ReLU}(x)\triangleq\max\{0,x\}$) with $\phi$ operating on a vector component-wise, $\mathrm{W}_\ell\in\mathbb{R}^{d_\ell\times d_{\ell-1}}$ is the weight matrix and $b_\ell\in\mathbb{R}^{d_\ell}$ is the bias. Fig.~\ref{FIG:noisy_neuron} shows a neuron in a noisy DNN.



%, and each hidden neuron has an independent Gaussian noise $\mathcal{N}(0,\beta^2)$ injected to its output. Each layer $\ell\in[0:L]$ is a high-dimensional random variable $T_\ell=\big(T_\ell(k)\big)_{k\in[d_\ell]}$ with values in $\mathbb{R}^{d_\ell}$.% The entries of $T_\ell$ are .% In a noisy DNNs the output of each neuron is perturbed by an independent Gaussian noise $\mathcal{N}(0,\beta^2)$, with $\beta$ being a design parameter tuned to produce both good classification performance and informative mutual information values.% We refer to such DNNs as \emph{noisy DNNs}.

%Formally, for $\ell\in[L]$, the $\ell$-th layer is described by $T_\ell=f_\ell(T_{\ell-1})+Z_\ell$, where $f_\ell:\mathbb{R}^{d_{\ell-1}}\to\mathbb{R}^{d_\ell}$ is a deterministic function of the previous layer and $Z_\ell\sim\mathcal{N}\big(0,\beta^2 I_{d_\ell}\big)$. To simplify notation, we set $S_\ell\triangleq f_\ell(T_{\ell-1})$. Our results do not rely on any particular~structure of $\{f_\ell\}_{\ell\in[L]}$, which can represent various types of layers (fully connected, convolutional, max-pooling, etc.). For instance, $T_\ell=\phi(\mathrm{W}_\ell T_{\ell-1}+b_\ell)+Z_\ell$ for fully connected or convolutional layers, where $\phi$ is the nonlinearity (e.g., $\tanh(x)$ or $\mathrm{ReLU}(x)\triangleq\max\{0,x\}$) with $\phi$ operating on a vector component-wise, $\mathrm{W}_\ell\in\mathbb{R}^{d_\ell\times d_{\ell-1}}$ is the weight matrix and $b_\ell\in\mathbb{R}^{d_\ell}$ is the bias. Fig.~\ref{FIG:noisy_neuron} shows a neuron in a noisy DNN.

% For fully connected layers $\mathrm{W}_\ell$ is arbitrary, while for convolutional layers $\mathrm{W}_\ell$ is Toeplitz.

%\ewout{Proposed text to replace above} The layers of a conventional DNN are described by $T_{\ell} = f_{\ell}(T_{\ell-1})$, with layer-specific transformations $f_{\ell}$. We generalize this to noisy DNNs where layers $\ell$ are defined by stochastic variables $S_{\ell} = f(T_{\ell-1})$ and $T_{\ell} = S_{\ell} + Z_{\ell}$ with $Z_{\ell} \sim\mathcal{N}(0,\beta_{\ell}^2 I)$ and $S_0 = X$. Unless stated otherwise we use $f_{\ell}(x) = \phi(\mathrm{W}_{\ell}x + b_{\ell})$, and set $\beta_0 = 0$ and $\beta_{\ell} = \beta$ for $\ell \geq 1$. Figure~\ref{FIG:noisy_neuron} shows a single neuron in a noisy DNN. Traditional DNNs are a special case where $\beta_{\ell} = 0$.

%\footnote{If the convolutional layer uses a kernel of size $q$, then $A_\ell(i+1,j+1)=A_\ell(i,j)$, for all $i\in[d_\ell]$ and $j\in[d_{\ell-1}]$, with $A_\ell(1,j)=a_\ell(j)$ when $j\in[q]$, and $A_\ell(1,j)=0$ otherwise.} 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{comment}
\begin{figure}[ht!]
	\begin{center}
	\includegraphics[width=0.4\textwidth]{NIPS2018/Figures/Miscellaneous/FigLayer.pdf}
		%\begin{psfrags}
		%	\psfragscanon
		%	\psfrag{A}[][][1]{\ \ \ \ \ \ $T_{\ell-1}$}
		%	\psfrag{B}[][][0.75]{$\phi\mspace{-3mu}\left(W_\ell^{(k)}T_{\ell-1}\mspace{-3mu}+\mspace{-3mu}b_\ell(k)\right)$}
		%	\psfrag{C}[][][1]{\ \ \ \ \ \ \ $S_\ell(k)$}
		%	\psfrag{D}[][][1]{\ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ $Z_\ell(k)\sim\mathcal{N}(0,\beta^2)$}
		%	\psfrag{E}[][][1]{$\mspace{-5mu}T_\ell(k)$}
		%	\includegraphics[scale = .7]{NIPS2018/Figures/Miscellaneous/Neuron.eps}
			\caption{$k$-th noisy neuron in a fully connected or a convolutional layer $\ell$.} \label{FIG:noisy_neuron}% with nonlinearity $\phi$; $\mathrm{W}_\ell^{(k)}$ and $b_\ell(k)$ are the $k$-th row and the $k$-th entry of the weight matrix and the bias vector,  respectively.} \label{FIG:noisy_neuron}
			%\psfragscanoff
		%\end{psfrags}
	\end{center}
\end{figure}
\end{comment}		


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%                                         %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%           Mutual Information            %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%                                         %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%\subsection{Mutual Information over Noisy DNNs}

%\final{shorten this! more to supplement about MI definition if needed.}


%Could break this into 2 subsections...Section 2.1 Characterization of DNN structure, Section 2.2 Mutual Information problem statement...

%The complicated structure of $P_{T_\ell|X}$  (due to the composition of Gaussian noises and nonlinearities) precludes an analytic computation of $I(X;T_\ell)$. .% This is the focus on the next section.



%. This map is a parametrized channel described by the conditional distribution $P_{T_1,\ldots,T_L|X}$, with network's weights and biases as the parameters. The corresponding probability density function\footnote{Due to the injection of Gaussian noise, given any $X=x$, $P_{T_1,\ldots,T_L|X=x}$ is absolutely continuous with respect to the Lebesgue measure.} (PDF) is $f_{T_1,\ldots,T_L|X=x}$. Its marginals are denoted by keeping only the relevant random variables in the subscript. 

%$\hat{P}_\mathcal{X}$ is assumed to be uniform over $\mathcal{X}$, i.e., $\hat{p}_\mathcal{X}(x)=\frac{1}{m}$, for all $x\in\mathcal{X}$. 

%\footnote{Viewing $\mathcal{X}$ as a collection of independently and identically distribution (i.i.d.) samples from a true distribution $P_X$, repetitions have zero probability under any reasonable model (common models assume the $P_X$ is smooth and concentrated on a low-dimensional Riemannian manifold in the high-dimensional ambient space).},



%from two main perspectives: (i) its evolution during training; (ii) its evolution throughout consecutive layers for fixed DNN parameters.


%\begin{remark}[Input Distribution Paradigm]\label{REM:Input_Dist_Paradigm}
%We adhere to the $X\sim\mathsf{Unif}(\mathcal{X})$ paradigm to conform with previous works on the topic \cite{DNNs_Tishby2017,DNNs_ICLR2018}. If instead one considers $X\sim P_X$, where $P_X$ is the true data distribution, a natural question is how the corresponding mutual information is related to \eqref{EQ:DNN_mutual_information}. In supplementary Section \ref{SUBSEC:two_MI_paradigms_relation} we relate the two quantities through a rigorous sample complexity bound.
%\end{remark}


% ==========================================================
% 2-Definitions
% ==========================================================

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%                                         %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%                Definition               %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%                                         %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%\subsection{Definitions}


% ==========================================================
% 3-Estimation
% ==========================================================

%However, generic estimates of differential entropy rely on restrictive assumptions of smoothness or boundness from above and below of the underlying PDF. Since we perturb the neurons with Gaussian noise (whose density has no lower bound above 0), our frameworks violates these assumptions. We circumvent these restrictions by developing a novel differential entropy estimator tailored for our particular scenario where $X$ and $T_\ell$ are connected through a noisy DNN.% We focus on the estimation of $h(f_{T_\ell})$; the process for estimating $h(f_{T_\ell}|X=x_i)$ is similar and explained in Subsection \ref{SUBSEC:Sample_prop_conditional_entropy}.

%Starting with $h(f_{T_\ell})$, 
%Since the noisy DNN is a directed generative model we may sample from $P_{T_\ell}$ and $P_{T_\ell|X}$ by forward-propagating randomly drawn samples from $P_X$ up the DNN. Expanding $I(X;T_\ell)$ as in \eqref{EQ:DNN_mutual_information}, it remains to estimate $h(f_{T_\ell})$ and $h(f_{T_\ell|X=x})$ for all $x\in\mathcal{X}$. 

%A direct approach for estimating $h(f_{T_\ell})$ would use samples from $T_\ell$ and a generic differential entropy estimator, however, the DNN has an additional layered structure where we know that $T_\ell = S_\ell + Z$ where $S_\ell$ is known and $Z$ is isotropic Gaussian noise with known parameters.
%e.g., 
%kNN-based \cite{jiao2017nearest} or KDE-based \cite{kandasamy2015nonparametric} estimators (see also references therein).


%Expanding $I(X;T_\ell)$ as in \eqref{EQ:DNN_mutual_information}, our goal is to estimate $h(p_{T_\ell})$ and $h(p_{T_\ell|X=x}),\ \forall x\in\mathcal{X}$. We develop a differential entropy estimator that leverages the ability to propagate samples up the layered structure and the known noise distribution. We call this estimator the \emph{sample propagation} (SP) estimator.

% As described next, an appropriate sampling procedure reduces estimating these conditional and unconditional entropies to a single new estimation problem: estimate $h(p_S\ast\varphi)$ based on i.i.d. samples $S^n\triangleq(S_i)_{i\in[n]}$ from $S\sim p_S$ and knowledge of $\varphi$. 

% After the reduction is established, we proposed an estimator for $h(p_S\ast\varphi)$, bound its estimation risk and propose an efficient methods for computing it. 

%Expanding $I(X;T_\ell)$ as in \eqref{EQ:DNN_mutual_information}, our goal is to estimate $h(p_{T_\ell})$ and $h(p_{T_\ell|X=x}),\ \forall x\in\mathcal{X}$. As described next, an appropriate sampling procedure reduces estimating these conditional and unconditional entropies to a single new estimation problem: estimate $h(p_S\ast\varphi)$ based on i.i.d. samples $S^n\triangleq(S_i)_{i\in[n]}$ from $S\sim p_S$ and knowledge of $\varphi$. After the reduction is established, we proposed an estimator for $h(p_S\ast\varphi)$, bound its estimation risk and propose an efficient methods for computing it. 

%\subsection{Sampling Procedure}

%\textbf{Unconditional Distribution:} For $h(p_{T_\ell})$, observe that since $T_\ell=S_\ell+Z_\ell$, where $S_\ell$ and $Z_\ell$ are independent, we have $p_{T_\ell}=p_{S_\ell}\ast \varphi$. To sample from $p_{S_\ell}$, let $\{\hat{x}_j\}_{j\in[n]}$ be $n$ i.i.d. samples from $P_X$. Feed each $\hat{x}_j$ into the DNN and collect the outputs it produces at the $(\ell-1)$-th layer. The function $f_\ell$ is then applied on each collected output to obtain $\mathcal{S}_\ell\triangleq\big\{s_{\ell,1},s_{\ell,2},\ldots,s_{\ell,n}\big\}$, which is a set of $n$ i.i.d. samples from $p_{S_\ell}$. 

%To estimate the mutual information in our stochastic DNN, we must estimate the conditional and unconditional entropies. 

%where the sample complexity is shows this estimation requires at least exponentially many samples in $d$.  %\kristjan{Should we justify the Gaussian mixture approach by connecting to literature on kernel based estimators?}
%\vspace{-2mm}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%          Gaussian Mixtures           %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%\vspace{-6mm}
%\subsection{Computing the Sample Propagation %Estimator}\label{SUBSEC:MoG_Entropy}

\begin{comment}
\begin{table}[ht]
    \begin{centering}
    \resizebox{\columnwidth}{!}{%
    \begin{tabular}{|c|c|}\hline
       \textbf{Lower Bounds}  & \textbf{Upper Bounds} \T\B\\\hline 
       $\frac{d}{2}\log\big(2\pi e \beta^2)$  & $\frac{d}{2}\log\big(2\pi e \beta^2)-\sum\limits_{i\in[n]}c_i\log c_i$\rule{0pt}{3ex}\rule[-2.8ex]{0pt}{0pt}\\\hline 
       $\frac{d}{2}\log(4\pi\beta^2)-\sum\limits_{i\in[n]}c_i\log\left(\sum\limits_{j\in[n]}c_je^{-\frac{\|\mu_i-\mu_j\|_2^2}{4\beta^2}}\right)$&
       $\begin{aligned}
       \frac{d}{2}\log\big(2\pi\beta^2\big)-\sum\limits_{i\in[n]}c_i\log\left(\sum\limits_{j\in[n]}c_je^{-\frac{\|\mu_i-\mu_j\|_2^2}{2\beta^2}}\right)
       \end{aligned}$ 
       \rule{0pt}{5.1ex}\rule[-3.6ex]{0pt}{0pt}\\\hline 
       $\frac{d}{2}\log\big(2\pi e \beta^2\big)-\sum\limits_{i\in[n]}c_i\log\left(\sum\limits_{j\in[n]}c_je^{-\frac{\|\mu_i-\mu_j\|_2^2}{8\beta^2}}\right)$&$\frac {1}{2}\logdet\left(2\pi e\sum\limits_{i\in[n]}c_i\mu_i\mu_i^\top-\mu\mu^\top+\beta^2 I_d\right)$   \rule{0pt}{4.6ex}\rule[-3.2ex]{0pt}{0pt}\\\hline
    \end{tabular}  
    }
    \end{centering}
    \caption{Bounds on the entropy of Gaussian mixtures, where $\mu\triangleq\sum_{i\in[n]}c_i\mu_i$ (bottom right).}\label{TABLE:Entropy_bounds}
\end{table}
\end{comment}

%is obtained by generating i.i.d. samples from $\hat{p}_{S_\ell} \ast \gamma$ and taking the empirical average of the log distribution $-\log (\hat{p}_{S_\ell} \ast \gamma)$, which is computed efficiently using optimized KDE algorithms. %with accuracy that scales as $1/\sqrt{n_\mathsf{MC}}$, where $n_\mathsf{MC}$ is the number of samples the algorithm uses. 
% <<<HERE>>>
%The estimate $\hat{h}_{\mathsf{SP}}$ is efficiently bounded above and below using bounds on the entropy of Gaussian mixtures. Table \ref{TABLE:Entropy_bounds} shows the bounds we use for $h(\sum_{i\in[n]} c_i \gamma_i)$, where $c_i\geq 0$ for all $i\in[n]$ and $\sum_{i\in[n]}c_i=1$, and each $\gamma_i$ is the PDF of $\mathcal{N}(\mu_i,\beta^2 \mathrm{I}_d)$. Proposition \ref{PROP:MoG_Entropy_Bounds} in Section \ref{SUPPSEC:Entropy_Bounds} in the supplement gives a full statement with a proof. None of these bounds imply one another and even in practice we found that none is consistently the tightest. We therefore adopt a greedy approach which computes all six estimates and uses the greatest lower bound and the least upper bound.


% ==========================================================
% 4-Examples
% ==========================================================

%The recent paper of Shwartz-Ziv and Tishby~\cite{DNNs_Tishby2017} concluded that DNN training consists of two distinct phases: an initial fitting phase and a subsequent compression phase that takes up most of the training time. A followup paper \cite{DNNs_ICLR2018} claimed that the compression observed in~\cite{DNNs_Tishby2017} is an artifact of the type of nonlinearities used in the DNN, rather than an inherent property of training. Specifically, the claim of \cite{DNNs_ICLR2018} was that double-sided saturating nonlinearities, such as tanh or sigmoid, compress, whereas single-sided saturating nonlinearities, such as ReLU, do not.
%An information-theoretic point of view explains the evolution of $I(X;T_\ell)$ during training. 

%\final{Igor - go over the text and suggest what can be shortened}

%even non-saturating nonlinearities such as leaky-ReLU can exhibit compression. An information-theoretic point of view fully explains the evolution of $I(X;T_\ell)$ as training progresses. 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%             Single-Layer Tanh
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%\subsection{Single Tanh Neuron}\label{SUBSEC:tanh_example}

%We track $I(X;T)$ as it evolves over training epochs, with
%\textbf{Single Neuron:} 

%\vspace{-3mm}



%
%
    %\centering


%\\
%    \small({\bf{d}}) & \small({\bf{e}}) & \small({\bf{f}})
%    \caption{Distribution of $R(X+b)+Z$ for: (a) two bias values and (b) behavior over a range of bias values; (c) network parameters of a two-layer ReLU network as a function of epoch; (d,e) the corresponding PDFs $f_{T_1(k)}$ and $f_{T_2(k)}$, and (f) the mutual information for both layers along with the lower and upper bounds obtained using the SP estimator.\ewout{combine/omit plots?}}\label{Fig:TwoLayerRelu}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%           Two-Layer LeakyReLU
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%\subsection{Two-layer leaky ReLU network}\label{SUBSEC:relu_example}


%\begin{figure}[h]
%\centering
%\begin{tabular}{cccc}
%\includegraphics[width=0.275\textwidth]{NIPS2018/Figures/Examples/FigReluBias.pdf} &
%\includegraphics[width=0.3\textwidth]{NIPS2018/Figures/Examples/FigReluT.png} &
%\includegraphics[width=0.29\textwidth]{NIPS2018/Figures/Examples/FigRelu2Param.pdf}%
%\begin{picture}(0,0)(0,0)\put(-102,69){\small({\bf{c}})}\end{picture} \\
%    \small({\bf{a}}) & \small({\bf{b}}) & \small({\bf{c}})\\
%\includegraphics[width=0.3\textwidth]{NIPS2018/Figures/Examples/FigRelu2DistT1.png}%
%\begin{picture}(0,0)(0,0)\put(-17,69){\small({\bf{d}})}\end{picture}&
%\includegraphics[width=0.3\textwidth]{NIPS2018/Figures/Examples/FigRelu2DistT2.png}%
%\begin{picture}(0,0)(0,0)\put(-100,67){\small({\bf{e}})}\end{picture} &
%\includegraphics[width=0.3\textwidth]{NIPS2018/Figures/Examples/FigRelu2MI.pdf}%
%\begin{picture}(0,0)(0,0)\put(-100,67){\small({\bf{f}})}\end{picture}
%\\
%    \small({\bf{d}}) & \small({\bf{e}}) & \small({\bf{f}})
%\end{tabular}
%\caption{Distribution of $R(X+b)+Z$ for: (a) two bias values and (b) behavior over a range of bias values; (c) network parameters of a two-layer ReLU network as a function of epoch; (d,e) the corresponding PDFs $f_{T_1(k)}$ and $f_{T_2(k)}$, and (f) the mutual information for both layers along with the lower and upper bounds obtained using the SP estimator.\ewout{combine/omit plots?}}\label{Fig:TwoLayerRelu}
%\end{figure}
\begin{comment}


\ewout{This 2nd example will probably have to move to the supplement}\\
\textbf{Two-Layer Leaky-ReLU Network:} Leaky-ReLU $R(x)\triangleq \max(x,x/10)$ has no saturation. Yet, we next show that a two-layer leaky-ReLU network can achieve compression. Let $\mathcal{X} = \mathcal{X}_0 \cup \mathcal{X}_{\nicefrac{1}{4}}$, with $\mathcal{X}_0 = \{1,2,3,4\}$ and $\mathcal{X}_{\nicefrac{1}{4}} = \{5,6,7,8\}$, and labels $0$ and $1/4$, respectively. We train the network via GD with learning rate 0.001 and mean squared loss. Initialization (shown in Fig. \ref{Fig:TwoLayerRelu}(a)) was chosen to best illustrate the connection between the Gaussians' motion and mutual information. 
%
The network converges to a solution where $w_1<0$ and $b_1$ is such that the elements in $\mathcal{X}_{\nicefrac{1}{4}}$ cluster. The output of the first layer is then negated using $w_2<0$ and the bias ensures that the elements in $\mathcal{X}_0$ are clustered without spreading out the elements in $\mathcal{X}_{\nicefrac{1}{4}}$. Figs.~\ref{Fig:TwoLayerRelu}(b) show the Gaussian motion at the output of the first layer and the resulting clustering. For the second layer (Fig.~\ref{Fig:TwoLayerRelu}(c)), the clustered bundle $\mathcal{X}_{\nicefrac{1}{4}}$ is gradually raised by growing $b_2$, such that its elements successively split as they cross the origin; further tightening of the bundle is due to shrinking $\vert w_2\vert$. Fig.~\ref{Fig:TwoLayerRelu}(d) shows the mutual information of the first (blue) and second (red) layers, and the estimated upper and lower bounds from Section~\ref{SEC:MI_estimation}. The merging of the elements in $\mathcal{X}_{\nicefrac{1}{4}}$ after their initial divergence is clearly reflected in the mutual information. Likewise, the spreading of the bundle, and successive splitting and coalescing of the elements in $\mathcal{X}_{\nicefrac{1}{4}}$ are visible in the spikes in the red mutual information curve. The figure also shows how the bounds on $I\big(X;T(k)\big)$ precisely track its evolution. 

\end{comment}

%Set $\mathcal{X}=\{1,2,3,4\}$ and note that the spacing between the points in $R(\mathcal{X}-b)$ is 1 for $b \leq 1$, and $1/10$ for $b \geq 4$. Thus, in the transition region between $1$ and $4$, some Gaussians move slower than others leading to gradual merging (Figs.~\ref{Fig:TwoLayerRelu}(a)-(b)).
%For any $x\in \mathcal{X}$ and linearly changing $b$, $x-b$ moves ten times slower when $x < b$ than when $x > b$. 



%We set initialization to encourage the network to find the desired solution where $w_1<0$ and $b_1$ is such that the elements in $\mathcal{X}_2$ compress. The output of the first layer is then negated using a negative $w_2$ and the bias is chosen so that the elements in $\mathcal{X}_1$ are clustered without spreading out the elements in $\mathcal{X}_2$.




% Instead of a single center we now convolve a transformed Gaussian with another Gaussian. 

% 0.6 compression: 54, 53, 51.5, 52




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%                                         
%%         Tanh vs ReLU Comparison
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%\subsection{Tanh versus ReLU Comparison}\label{SUBSEC:tanh_relu_compare}

%\textbf{Tanh vs. ReLU Comparison:} The primary difference between double-sided saturating activations and single-sided or non-saturating ones is that the former often allow a long, gradual reduction of the loss as the weights grow. Single-sided or non-saturating activations lack this mechanism, making the compression in $I(X;T)$ occur over a much shorter interval than in the double-sided case.% function than for non-saturating ones.

%\begin{figure}[h]
%\end{figure}

%\ewout{This paragraph is based on figure 7 and 15 in the menu. The non-present figures I'm referring to are the zoomed out MI and Gaussian motions in both cases. Numbering is (a) MI for tanh; (b) Gaussians for tanh; (c) MI for leaky-ReLU; (d) Gaussians for leaky-ReLU.}

%We highlight the main difference between the evolution of $I\big(X;T(k)\big)$ during training under tanh and (Leaky) ReLU architectures. Fig. \ewout{add figure of tanh vs relu MI and Gaussian movement where x axis is zoomed out, i.e., for many training epochs.} shows $I\big(X;T(k)\big)$ and the corresponding motion of Gaussians for two single-layer examples (similar to Section \ref{SUBSEC:tanh_example}), one with tanh nonlinearity and the other with leaky-ReLU. In both cases, the mutual information swiftly rises at the beginning of training. For the tanh network (Figs. \ref{ref}(a)), $I\big(X;T(k)\big)$ then slowly decrease during the entire $~9.5\cdot 10^4$ remaining training epochs. To the contrary, when leaky-ReLU is used, after the initial rise the mutual information drops to its lowest value at around $10^4$ epochs and essentially stays constant (and even mildly rises) from that point and beyond.


%To understand why tanh networks can keep compressing for a long time, while ReLU networks present a swift compression consider Figs. \ref{ref}(b) and \ref{ref}(d). The tanh network can keep pushing the two clusters while moving the Gaussians in the bottom cluster closer together to improve classification. This exploits the saturation regime of tanh and achieved by increasing the weight and adjusting the bias (so that the tanh middle point stays in between the two clusters). The improved clustering of the three bottom Gaussians makes them increasingly indistinguishable and causes the slow reduction in $I\big(X;T(k)\big)$ observed in Fig. \ref{ref}(a). For leaky-ReLU, on the other hand, once the bias is in place after roughly $10^4$ epochs, the classes are separated and significantly tweaking the parameters further is not beneficial. For instance, a large increase of the weight would push the clusters further apart but would also separate the Gaussians in the bottom cluster. This tradeoff stabilizes the system (as seen in Fig. \ref{ref}(b) from epoch $\sim 2\cdot10^4$ and beyond), and keep the mutual information roughly fixed. 


% This information rate corresponds to how distinguishable are the channel's inputs (namely, the elements of $\mathcal{S}_k$) when composed with Gaussian noise. To understand this, note that the distribution of the channel's output $S(k)+Z$ is a mixture of Gaussians with means at the points $s\in\mathcal{S}_k$. The closer two constellations points are, the more overlapping the corresponding Guassians at the output. Consequently, it becomes harder to distinguish these two constellation points if either is transmitted, which causes the mutual information to drop. 


% We first illustrate this idea using some small examples; the next section shows that the motion of
% Gaussians drives the behavior of $I\big(X;T(k)\big)$ for larger DNNs as well.

%As explained in the introduction, tracking $I(X;T_\ell)$, where $\ell\in[L]$, during training or %throughout layers makes little sense for deterministic DNNs because its true value is just the %constant $H(X)$. For noisy DNNs, on the other hand, the question of how $I(X;T_\ell)$ evolves during %training becomes meaningful, and our goal is to understand under what conditions does compression %happen.  

%As the following minimal examples illustrate, compression is possible regardless of whether %double-sided nonlinearities are employed or otherwise. Furthermore, we adopt an information-theoretic %point of view that fully explains the various trends the mutual information $I(X;T_\ell)$ presents %(peaks, drops, compresses, etc.). We start with the simple case of a noisy shallow neural network %(SNN) with single input and output neurons. The setup is shown in Fig. \ref{FIG:noisy_neuron} for %$\ell=L=d_0=d_1=1$. Throughout this section we assume that $\sigma$ is an invertible map. Hence instead %of $\mathsf{ReLU}$ we consider $\mathsf{leaky-ReLU}(x)\triangleq\max\left\{x,-\frac{x}{20}\right\}$; %since $\mathsf{leaky-ReLU}$ does not saturate on either side, according to \cite{DNNs_ICLR2018} it %should not compress. 


%\subsection{Double-Sided Saturating Nonlinearity}\label{SUBSEC:Examples_Tanh}

%Assume that $\sigma=\tanh$, let the labeled data set be $\left\{(-1,-1),\left(-\frac{1}{3},-1\right),\left(\frac{1}{3},-1\right),(1,1)\right\}$ and set $\beta=0.05$. Namely, there are 4 data point ($\left\{\pm\frac{1}{3},\pm1\right\}$) separated into two classes ($-1$ and $+1$)\footnote{Equivalently, one may consider $\sigma=\mathrm{sigmoid}$ and relabel the $-1$ class as $0$.}. This gives $\mathcal{X}=\left\{\pm\frac{1}{3},\pm1\right\}$ and $$\mathcal{S}_k=\bigg\{\tanh(-w_k+b_k),\tanh\left(-\frac{w_k}{3}+b_k\right),\tanh\left(\frac{w_k}{3}+b_k\right),\tanh(w_k+b_k)\bigg\}.$$ Intuitively, a good classifier $T(k)=\tanh(w_kX+b_k)+Z$ for this data should set the 0 of the nonlineariy anywhere between $\frac{1}{3}$ and $1$ and push the weight $w$ high enough to sharpen the threshold. \ewout{Please add a sentence or two about how training was done} We trained this small SNN via...

%\ewout{When the final plots are added, descriptions of at what approximate epoch (i.e., values of $k$) each effect happens should added to the following paragraph (see specific comments below). The current labels of the subfigures might need to change too}

%As expected and shown in Fig. \ref{FIG:Tanh_Example}(a), the weight monotonically grows as training progresses, while the bias tends to $-\frac{2}{3}w_k$, setting the right threshold. The effect this has on the Gaussian mixture $S(k)+Z$ is illustrated in Fig. \ref{FIG:Tanh_Example}(b), where the vertical axis is a heatmap of the four Gaussians at each epoch and the horizontal axis is $k\in[10^5]$. Fig. \ref{FIG:Tanh_Example}(c) zooms in the first $10^4$ training epochs. These figures show the clustering our classifier imposes on these Gaussians (moving the 3 point labeled $-1$ closer together and pushing the $+1$ labeled data point further away). Looking at the mutual information plots in Figs. \ref{FIG:Tanh_Example}(e)-(f), the expected effect of the coalescing Gaussian on $I\big(X;T(k)\big)$ is clear. Training is initiated at $b_0=w_0=0$, whence the four points in $\mathcal{S}_0$ coincide at 0 and the mutual information is 0 (as $S(0)=0$ is a constant). When $b_k$ is still close to zero but $w_k$ begins to grow, the four Gaussians separate (which corresponds to $\mathcal{S}_k$ becoming an increasingly better constellation for transmitting 4 possible values over the AWGN channel) causing $I\big(X;T(k)\big)$ to rise \ewout{When does it peak? Why there (bias/weight)?}. As training progresses, the three bottom Gaussians come closer and closer together. This pushes $\mathcal{S}_k$ towards becoming a binary constellation and produces the compression phase of $I\big(X;T(k)\big)$ \ewout{Starting from which epoch? Does it stabilize? Why?}.\\


%\begin{figure}[t!]
%	\begin{center}
%    \subfloat[]{\includegraphics[scale=0.5]{NIPS2018/Figures/Examples/Tanh_bias_weight_loss.eps}}\\
%    \subfloat[]{\includegraphics[scale=0.4]{NIPS2018/Figures/Examples/Tanh_Gaussians_all.eps}}\quad\quad
%    \subfloat[]{\includegraphics[scale=0.4]{NIPS2018/Figures/Examples/Tanh_Gaussians_begin.eps}}\\
%    \subfloat[]{\includegraphics[scale=0.3]{NIPS2018/Figures/Examples/Tanh_MI_all.eps}}\quad\quad
%    \subfloat[]{\includegraphics[scale=0.3]{NIPS2018/Figures/Examples/Tanh_MI_log.eps}}
%	\caption{\ewout{These are all placeholder plots: Please replace with final versions} Double-sided saturating nonlinearity ($\sigma=\tanh$): (a) Bias/weight/loss evolution - bias and weight, respectively, decrease and increase tending to a ratio of $-\frac{2}{3}$, which places the $\tanh$'s threshold between the two classes; (b)-(c) Motion of Gaussian at the output - as training progresses, the three $-1$ labeled Gaussians get clustered together, while the $+1$ labeled one is pushed apart from them; (d)-(e) Mutual information evolution - numerical computation of $I\big(X;T(k)\big)$ versus the training epochs ($k\in[10^5]$ for (d) and $k\in[10^4]$ for (e)). Initially, the Gaussians are spread apart (as $w_k$ grows from 0 and $b_k$ is relatively close to 0) thus making them more distinguishable, which increases mutual information. As $b_k$ approaches $-\frac{2}{3}$ (and $w_k$ keeps growing), the three bottom Gaussians coalesce causing the mutual information to drop.} \label{FIG:Tanh_Example}
%    \end{center}
%\end{figure}
		

%\subsection{Non-Saturating Nonlinearity}\label{SUBSEC:Examples_ReLU}

%\ewout{Ewout, I didn't go into it but this should probably be added: We should make the point discussed today at the Slack chat why ReLU compresses fast and stabilizes while tanh/sigmoid keep on going...}


%We next shown that similar effects happens even when $\sigma$ is non-saturating. Let $\sigma=\mathsf{leaky-ReLU}$ and consider the same set up as before but with the label $0$ instead of $-1$. This time we initiate training at $w_0=0$ and $b_0=3$, which places the $\mathsf{LeakyReLU}$'s middle point to the left of the entire data set. The classifier should push $b_k$ rightwards to any point between $\frac{1}{3}$ and $1$ and increase $w_k$. Fig. \ref{FIG:ReLU_Example}(a) confirms that this indeed happens during training.

%The effect this has on the Gaussian mixture $S(k)+Z$ and the mutual information $I\big(X:T(k)\big)$ is shown in Figs. \ref{FIG:ReLU_Example}(b)-(e) and described as follows. At first, all four Gaussians are in the large-slope regime of the $\mathsf{LeakyReLU}$ (i.e., on its RHS). As long as this is the case, growing $w_k$ pushes the Gaussians away from each other and increases $I\big(X;T(k)\big)$ (until approximately $k=1.5\cdot10^3)$. Then, $b_k$ goes below $\frac{1}{3}$, which mean that the two left-most Gaussians are in the low-slope regime of the non-linearity. The small slope of $\frac{1}{20}$ essentially merges these two Gaussians, which is shrinks the number of distinguishable symbols in $\mathcal{S}_k$ from 4 to 3. At this time, $I\big(X;T(k)\big)$ presents its first dip. The second dip of mutual information occurs at roughly $k=7.5\cdot 10^3$, which is when $b_k$ goes below $-\frac{1}{3}$. This means that the third Gaussian enters the low-slope region as well and merges with the two Gaussians that were already there. Then $b_k$ stabilizes, holding the two clusters separated for all subsequent epochs. \ewout{For some reason, the placeholding plots appear at the bottom of the document. Please make sure they are in the right place one the final version are added}

%While the mutual information dynamics appear less smooth for $\mathsf{LeakyReLU}$ than for $\tanh$, both cases present a gradual decrease in $I\big(X;T(k)\big)$ as $k$ progresses. This implies that compression of mutual information in not an artifact of the particular properties of the employed nonlinearity (double-sided saturation or not). Rather, it is a consequence of the clustering preformed by the neural network. Clustering inputs corresponds to a smaller number of distinguishable AWGN channel outputs, and hence, a lower information rate. 


%\begin{figure}[t!]
%	\begin{center}
    %\subfloat[]{\includegraphics[width=1in]{NIPS2018/Figures/Examples/ReLU_bias_weight_loss.eps}}\quad 
    %\subfloat[]{\includegraphics[width=1in]{NIPS2018/Figures/Examples/ReLU_Gaussians_all.eps}}\quad\quad
    %\subfloat[]{\includegraphics[width=1in]{NIPS2018/Figures/Examples/ReLU_Gaussians_begin.eps}}\\
    %\subfloat[]{\includegraphics[width=5in]{NIPS2018/Figures/Examples/ReLU_MI.eps}}
%	\caption{\ewout{These are placeholding plots. Here I used Setting=6 (the low slope is 1/20 there). I think for ReLU it suffices to run up to, say, $2\cdot 10^4$ epochs since nothing interesting really happens afterwards} Non-saturating nonlinearity ($\sigma=\mathsf{LeakyReLU}$): (a) Bias/weight/loss evolution - bias decreases pushing the middle point of the nonlinearity in between $\frac{1}{3}$ and 1; the increase in weight sharpens the threshold. (b)-(c) Motion of Gaussian at the output - the three $-1$ labeled Gaussians are clustered together by moving the bias from the initial $b_0=3$ to $\approx\frac{1}{2}$. (d)-(e) Mutual information evolution - numerical computation of $I\big(X;T(k)\big)$ versus the training epochs ($k\in[10^5]$ for (d) and $k\in[10^4]$ for (e)). Initially, the Gaussians are all at the large-slope regime of the nonlinearity. As long as $b_k>1$, the increase in $w_k$ spreads the Gaussians further apart and grows mutual information. When $b_k<\frac{1}{3}$ (at approximately $k=1.5\cdot 10^3$) the two bottom Gaussians are merged and the first drop in $I\big(X;T(k)\big)$ occurs. Further lowering the bias to $b_k<-\frac{1}{3}$ (at around $k=7.5\cdot 10^3)$ merges the 3rd Gaussians with the bottom two that have already merged. This produces the 2nd drop in mutual information. Afterwards the system stabilizes and  $I\big(X;T(k)\big)$ roughly remains constant.} \label{FIG:ReLU_Example}
%    \end{center}
%\end{figure}
		
%\subsection{The Effect of Noise Level}\label{SUBSEC:Examples_Noise_Level}

%\begin{figure}[!ht]
%	\begin{center}
	    %\subfloat[]{\includegraphics[width=2in]{NIPS2018/Figures/Examples/plotMI_Sigmoid.eps}}\quad %\subfloat[]{\includegraphics[width=3in]{NIPS2018/Figures/Examples/Fat_Gaussians.eps}}
%		\caption{(a) The mutual information $I\big(X;\sigma(wX+b)+Z\big)$, for $w\in[0,20]$, $b=-\frac{2}{3}w$ and different $\beta^2$ values. (b) PDF of the Gaussian mixture $\sigma(wX+b)+Z$ for $Z\sim\mathcal{N}(0,0.2^2)$ - the three bottom Gaussians are indistinguishable for the beginning. Hence, clustering causes no mutual information drop and compression disappears. \ewout{Placeholding plot. Suggested modifications/additions for final version: Subfigure (a) - this figure is for sigmoid and should be re-plotted for tanh; making the lines thicker and add a legend. Subfigure (b) - I used trainTanhPlot(1) function but changes beta to 0.2 (variance is $0.2^2$); this corresponds to the green curve in Subfigure (a)} }\label{FIG:MI_different_noise}
%    \end{center}
%\end{figure}

%Our next focus is the effect of $\beta^2$ on $I\big(X;T(k)\big)$. From the AWGN communication channel perspective, the higher $\beta^2$ (noise level) is, the lower should the information rate be. However, growing $\beta^2$ from small to large reveals an additional intriguing phenomena intimately related to compression. To illustrate we go back to the double-sided saturating case from Section \ref{SUBSEC:Examples_Tanh} (however, the same holds for the non-saturating scenario as well). 


%Section \ref{SUBSEC:Examples_Tanh} illustrates that training evolves the weight and bias in such a way that $\frac{b_k}{w_k}\to \frac{2}{3}$. To isolate the effect of the noise level on the mutual information, we set $b=-\frac{2}{3}w$ and plot $I\big(X;\sigma(wX+b)\big)$ for $w\in[0,20]$ for different values of $\beta\in\{0.01, 0.02, 0.05, 0.1, 0.2, 0.5\}$. The curves are shown on Fig. \ref{FIG:MI_different_noise}(a), which reveals that for high enough noise variance compression is impossible in this setup (as long as $w$ keeps growing during training). To see why, Fig. \ref{FIG:MI_different_noise}(b) shows that Gaussian motion from Fig. \ref{FIG:Tanh_Example}(b) but when $\beta=0.2$ (rather than the $\beta=0.05$ used therein). With this high noise parameter, the three bottom Gaussians (which correspond to the $-1$ labeled inputs $\left\{-1,-\frac{1}{3},\frac{1}{3}\right\}$) are effectively merged from the beginning, even when their means are relatively separated. The classifier grows $w$, which pushes these means closer together in order to clusters the corresponding inputs. However, since they were indistinguishable to begin with, this doesn't cause the mutual information to drop because. The gradual increase in mutual information is due to the improved separation between the two classes as $w$ grows. From the communication perspective, $\mathcal{S}_k$ is a binary constellation for all $w_k$ values, but growing $w$ makes it a better binary constellation since its two symbols become increasingly separated. As shown in the next section, a similar dependence on the noise parameter is observed for larger DNNs as well. Namely, growing $\beta$ sufficiently high make every trace of compression disappear. 


%\subsection{Two-Layered Example}\label{SUBSEC:Examples_Two_Layers}

%\ewout{Please decide if there is an added value to the two-layered example and add it if you see fit. Presentation should be similar to the above, but probably more concise (since the ideas are established by now)}


==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    # if the dependency isn't one of the files that this latexmk run will consider, process it
    # without this test, we would get an infinite loop!
    if (!($root_filename eq $_[0]))
    {
        system( "latexmk -pdf \"$_[0]\"" );
    }
}

==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak

